The Cosmological Parameters 2014

This is a review article for The Review of Particle Physics 2014 (aka the Particle Data Book). It forms a compact review of knowledge of the cosmological parameters at the beginning of 2014. Topics included are Parametrizing the Universe; Extensions to the standard model; Probes; Bringing observations together; Outlook for the future.

==> hubble-allref.tex <==
% This version 02/11/13 
 
\referencelist 
 
\reference{planckI} P.A.R. Ade \etal\ (Planck Collaboration 2013 I), arXiv:1303.5062v1
\endreference
 
\reference{planckXVI} P.A.R. Ade \etal\ (Planck Collaboration 2013 XVI), arXiv:1303.5076v1
\endreference
 
\reference{wmap9be} C. Bennett \etal, to appear, Astrophys. J. Supp., arXiv:1212.5225v3
\endreference 
 
\reference{wmap9hi} G. Hinshaw \etal, to appear, Astrophys. J. Supp., arXiv:1212.5226v3
\endreference 
 
\reference{solosc} S. Fukuda \etal, \prl85,3999(2000)  
\endreference 
 
\reference{*xxx} Q.R. Ahmad \etal, \prl87,071301(2001) 
\endreference 
 
\reference{inf} E.W. Kolb and M.S.  
	Turner, {\it The Early Universe}\rm, Addison--Wesley (Redwood City, 1990) 
\endreference 
 
\reference{PDP} D.H. Lyth and A.R. Liddle, {\it The Primordial Density 
Perturbation}\rm, Cambridge University Press (2009) 
\endreference 

\reference{LL}
A.R. Liddle and D.H. Lyth, \plB291,391(1992)
\endreference
 
\reference{Boltz} A. Lewis, A Challinor, and A. Lasenby, \aj538,473(2000)    
\endreference 
 
\reference{*xxx}  D. Blas, J. Lesgourgues, and T. Tram, JCAP {\bf 1107}, 034 (2011)   
\endreference 
  
\reference{fix} D. Fixsen, \aj707,916(2009) 
\endreference 
 
\reference{KT} A. Kosowsky and M.S. Turner, \prD52,1739(1995) 
\endreference 
 
\reference{mw} K.A. Malik and D. Wands, \prept475,1(2009) 
\endreference 
 
\reference{planckXXV} P.A.R. Ade \etal\ (Planck Collaboration 2013 XXV), arXiv:1303.5085v1
\endreference 
 
\reference{curv} D.H. Lyth and D. Wands, \plB524,5(2002)  
\endreference 
 
\reference{*xxx} K. Enqvist and M.S. Sloth, \npB626,395(2002)
\endreference 
 
\reference{*xxx} T. Moroi and T. Takahashi, \plB522,215(2001)
\endreference 
 
\reference{man05}  G. Mangano, G. Miele, S. Pastor, T. Pinto, O. Pisanti, and P.D. Serpico, \npB729,221(2005)
\endreference
 
\reference{Neff}  S. Riemer-S{\o}rensen, D. Parkinson, and T.M. Davis, PASA {\bf 30}, e029 (2013)
\endreference
 
\reference{Webb} J.K. Webb \etal, \prl107,191101(2011)
\endreference 
 
\reference{*xxx} J.A. King \etal, \mnras422,3370(2012) 
\endreference 
 
\reference{*xxx} P. Molaro \etal, \aap555,68(2013)  
\endreference 

\reference{planckXXVI} P.A.R. Ade \etal (Planck Collaboration 2013 XXVI), arXiv:1303.5086v1
\endreference
 
\reference{freedman} W.L. Freedman \etal, \aj553,47(2001) 
\endreference 
 
\reference{riess09} A.G. Riess  \etal, \aj730,119 (2011) 
\endreference 
 
\reference{leibundgut} B. Leibundgut, \araa39,67(2001)  
\endreference 
 
\reference{snfirst} A.G. Riess \etal, Astron.\ J.\ {\bf 116}, 1009 (1998) 
\endreference 
 
\reference{*xxx} P. Garnavich \etal, \aj509,74(1998) 
\endreference 
 
\reference{*xxx} S. Perlmutter \etal, \aj517,565(1999)
\endreference 
 
\reference{SNLS3} A. Conley \etal, \ajs192,1(2011)   
\endreference 
 
\reference{*xxx} M. Sullivan \etal, \aj737,102(2011) 
\endreference 
 
\reference{kowalski} M. Kowalski  \etal, \aj686,749(2008) 
\endreference 
 
\reference{kessler} R. Kessler  \etal, \ajs185,32(2009) 
\endreference 
 
\reference{LewBrid} A. Lewis and S. Bridle, \prD66,103511(2002) 
\endreference 
 
\reference{DASI} J. Kovac \etal, \nature420,772(2002)
\endreference 
 
\reference{Das} S. Das \etal, \prl107,021301(2011) 
\endreference 
 
\reference{eisenstein05} D. Eisenstein  \etal, \aj633,560(2005) 
\endreference 
 
\reference{cole05} S. Cole  \etal, \mnras362,505(2005) 
\endreference 
 
\reference{boss13} A. Sanchez \etal, arXiv:1303.4396
\endreference 
 
\reference{parkinson13} D. Parkinson \etal, arXiv:1210.2130
\endreference 
 
\reference{blake11} C. Blake  \etal, \mnras418,1707(2011) 
\endreference 
 
\reference{kaiser} N. Kaiser, \mnras227,1(1987) 
\endreference 
 
\reference{guzzo} L.  Guzzo \etal, \nature451,541(2008) 
\endreference 
 
\reference{nusser11} A. Nusser and M. Davis, \aj736,93(2011) 
\endreference 

\reference{blake12} C. Blake \etal, arXiv:1204.3674
\endreference

\reference{isw1} R.G. Crittenden and N. Turok, \prl75,2642(1995) 
\endreference 
 
\reference{tg13} T. Giannatonio, R.  Crittenden, R. Nichol, and A. Ross, \mnras426,258(2012)
\endreference

\reference{planckXIX} P.A.R. Ade \etal\ (Planck Collaboration 2013 XIX), arXiv:1303.5076v1
\endreference

\reference{lp06} J. Lesgourgues and  S. Pastor, \prept429,307(2006) 
\endreference 
 
\reference{thomas10} S. Thomas, F.B. Abdalla, and O. Lahav, 
\prl105,031301(2010)  
\endreference 
  
\reference{boss_nu12} G.-B. Zhao  \etal,  MNRAS, doi:10.1093/mnras/stt1710 (early on-line)
\endreference

\reference{wigglez_nu12} S. Riemer-S{\o}rensen \etal, \prD85,081101(2012) 
\endreference

\reference{planckXX} P.A.R. Ade \etal\ (Planck Collaboration 2013 XX), arXiv:1303.5080v1
\endreference 
   
\reference{slosar13}
 A. Slosar \etal,  arXiv:1301.3459
\endreference

\reference{viel13}
M. Viel \etal,  arXiv:1306.2314
\endreference

\reference{lensing}  A. Refregier, \araa41,645(2003) 
\endreference 
 
\reference{*xxx} R. Massey \etal, \nature445,286(2007) 
\endreference 
 
\reference{*xxx} H. Hoekstra and B. Jain, \arnps58,99(2008) 
\endreference 
 
\reference{cfhtlens13} M. Kilbinger \etal, \mnras430,2200(2013)
\endreference
 
\reference{*xxx} C. Heymans \etal, \mnras427,146(2012)
\endreference

\reference{dekel} A. Dekel, \araa32,371(1994) 
\endreference 
 
\reference{planckXXIV} P.A.R. Ade \etal\ (Planck Collaboration 2013 XXIV), arXiv:1303.5084v1
\endreference 

\endreferencelist 


==> hubble-body.tex <==
\BleederPointer=7
\font\tencaps=cmcsc10

%
% Revised 29 Oct  2013  12noon
%---------------------------
\IndexEntry{hubblepage}
\heading{THE COSMOLOGICAL PARAMETERS}
%Redefine upper case greek letters so that particle names are slanted
%Make new definitions to correspond to old definitions
\mathchardef\OMEGA="700A

\beginRPPonly
\runninghead{The Cosmological Parameters}
\IndexEntry{hubbleCosmParam}

\def\paragraph#1{\medskip\noindent\bgroup\boldface\bfit #1:\egroup}
\def\mnras#1,#2(#3){{\rm MNRAS\ }{\bf #1}, {\rm#2} {\rm(#3)}}

\overfullrule=5pt

\ifnum\WhichSection=7
\magnification=\magstep1
\fi

%Redefine upper case greek letters so that particle names are slanted
%Make new definitions to correspond to old definitions
\mathchardef\OMEGA="700A
\mathchardef\OMEGA="700A
\WhoDidIt{Updated November 2013, by O.~Lahav (University College London) % 
and A.R.~Liddle (University of Edinburgh).}%\WhoDidIt

%% \def\kmsMpc{km~s$^{-1}$~Mpc$^{-1}$}



\ifnum\WhichSection=7
\else
\advance\baselineskip by -.2pt
\fi

\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\simlt{\lower.5ex\hbox{\ltsima}} \def\gtsima{$\; \buildrel > \over
\sim \;$} \def\simgt{\lower.5ex\hbox{\gtsima}}

\section{Parametrizing the Universe}

Rapid advances in observational cosmology have led to the
establishment of a precision cosmological model, with many of the key
cosmological parameters determined to one or two significant figure
accuracy. Particularly prominent are measurements of cosmic microwave
background (CMB) anisotropies, with the highest precision observations being those of the {\it Planck} Satellite\cite{planckI}\cite{planckXVI} which for temperature anisotropies supersede the iconic {\it WMAP} results\cite{wmap9be}\cite{wmap9hi}. However the most accurate
model of the Universe requires consideration of a range of
different types of observation, with complementary probes providing
consistency checks, lifting parameter degeneracies, and enabling the
strongest constraints to be placed.

The term `cosmological parameters' is forever increasing in its scope,
and nowadays often includes the parameterization of some functions, as well
as simple numbers describing properties of the Universe. The original
usage referred to the parameters describing the global dynamics of the
Universe, such as its expansion rate and curvature. Also now of great
interest is how the matter budget of the Universe is built up from its
constituents: baryons, photons, neutrinos, dark matter, and dark
energy. We need to describe the nature of perturbations in the
Universe, through global statistical descriptors such as the matter
and radiation power spectra. There may also be parameters describing
the physical state of the Universe, such as the ionization fraction as
a function of time during the era since recombination.  Typical
comparisons of cosmological models with observational data now feature
between five and ten parameters.

\subsection{The global description of the Universe}

Ordinarily, the Universe is taken to be a perturbed Robertson--Walker
space-time with dynamics governed by Einstein's equations. This is
described in detail by Olive and Peacock in this volume.
\IndexEntry{hubbleFracDensity}\IndexEntry{hubbleCosmConLam}Using the 
density parameters $\OMEGA_i$ for the various matter species and
$\OMEGA_\LAMBDA$ for the cosmological constant, the Friedmann equation
can be written
$$
\sum_i \OMEGA_i + \OMEGA_\LAMBDA -1 = \frac{k}{R^2 H^2} \,,
\EQN{redfried}
$$
where the sum is over all the different species of material in the
Universe. This equation applies at any epoch, but later in this
article we will use the symbols $\OMEGA_i$ and $\OMEGA_\LAMBDA$ to
refer to the present values.  

The complete present state of the homogeneous Universe can be
described by giving the current values of all the density parameters
and the Hubble constant $h$ (the present-day Hubble parameter being written $H_0 = 100 h \, {\rm km}\,{\rm s}^{-1}\,{\rm Mpc}^{-1}$).  A typical collection would be baryons $\OMEGA_{{\rm b}}$,
photons $\OMEGA_\gamma$, neutrinos $\OMEGA_\nu$, and cold dark matter $\OMEGA_{{\rm c}}$ (given charge neutrality, the
electron density is guaranteed to be too small to be worth considering
separately and is included with the baryons). \IndexEntry{hubbleMassDens}\IndexEntry{hubbleDM}\IndexEntry{hubbleBaryon}
The spatial curvature can then be determined from the other parameters using
\Eq{redfried}. 
The total present matter density $\OMEGA_{{\rm m}}
=\OMEGA_{{\rm c}}+\OMEGA_{{\rm b}}$ is sometimes used in place of the
cold dark matter density $\OMEGA_{{\rm c}}$.

\newpage % New page forced by hand as otherwise page 1 is over length for some reason.

These parameters also allow us to track the
history of the Universe back in time, at least until an epoch where
interactions allow interchanges between the densities of the different
species, which is believed to have last happened at neutrino
decoupling, shortly before Big Bang Nucleosynthesis (BBN).  To probe
further back into the Universe's history requires assumptions about
particle interactions, and perhaps about the nature of physical laws
themselves.

%\subsection{Neutrinos}

%\labelsubsection{neut}

The standard neutrino sector has three flavors. For neutrinos of mass
in the range $5 \times 10^{-4} \, {\rm eV}$ to $1\,{\rm MeV}$, the
density parameter in neutrinos is predicted to be
$$
\OMEGA_\nu h^2 = \frac{\sum m_\nu}{93 \, {\rm eV}} \,,
\EQN{}
$$
where the sum is over all families with mass in that range (higher
masses need a more sophisticated calculation). We use units with $c=1$
throughout. Results on atmospheric and Solar neutrino
oscillations\cite{solosc} imply non-zero mass-squared differences
between the three neutrino flavors.  These oscillation experiments
cannot tell us the absolute neutrino masses, but within the simple
assumption of a mass hierarchy suggest a lower limit of approximately
$0.06$ eV\IndexEntry{hubbleNuDens} on the sum of the neutrino masses.

Even a mass this small has a
potentially observable effect on the formation of structure, as
neutrino free-streaming damps the growth of perturbations. Analyses commonly now either assume a neutrino mass sum fixed at this lower limit, or allow the neutrino mass sum as a variable parameter. To date there is no decisive evidence of any
effects from either neutrino masses or an otherwise non-standard
neutrino sector, and observations impose quite stringent limits, which we summarize
in \Section{neut2dF}.  However, we note that the inclusion of the neutrino
mass sum as a free parameter can affect the derived values of other
cosmological parameters.

%The cosmological effect of neutrinos can also be modified if the
%neutrinos have decay channels, or if there is a large asymmetry in the
%lepton sector manifested as a different number density of neutrinos
%versus anti-neutrinos. This latter effect would need to be of order
%unity to be significant (rather than the $10^{-9}$ seen in the baryon
%sector), which may be in conflict with nucleosynthesis\cite{dol}.
%
\subsection{Inflation and perturbations}
\IndexEntry{hubbleInflation}

A complete model of the Universe should include a description of
deviations from homogeneity, at least in a statistical way. Indeed,
some of the most powerful probes of the parameters described above
come from the evolution of perturbations, so their study is naturally
intertwined in the determination of cosmological parameters.

There are many different notations used to describe the perturbations,
both in terms of the quantity used to describe the perturbations and
the definition of the statistical measure. We use the dimensionless
power spectrum $\Delta^2$ as defined in Olive and Peacock (also
denoted ${\cal P}$ in some of the literature). If the perturbations
obey Gaussian statistics, the power spectrum provides a complete
description of their properties.

From a theoretical perspective, a useful quantity to describe the
perturbations is the curvature perturbation ${\cal R}$, which measures
the spatial curvature of a comoving slicing of the space-time.  A simple case
is the
\IndexEntry{hubbleHZeldovich}Harrison--Zel'dovich spectrum, which
corresponds to a constant $\Delta^2_{{\cal R}}$. More generally, one
can approximate the spectrum by a power-law, writing
$$
\Delta^2_{{\cal R}}(k) = \Delta^2_{{\cal R}}(k_*) 
\left[\frac{k}{k_*}\right]^{n_{{\rm s}}-1} \,,
\EQN{}
$$
where $n_{{\rm s}}$ is known as the spectral index, always defined so that $n_{{\rm s}}=1$
for the Harrison--Zel'dovich spectrum, and $k_*$ is an arbitrarily
chosen scale.  The initial spectrum, defined at some early epoch of
the Universe's history, is usually taken to have a simple form such as
this power-law, and we will see that observations require $n_{{\rm s}}$ close to
one. Subsequent evolution will modify the spectrum
from its initial form.

The simplest mechanism for generating the observed
perturbations is the inflationary cosmology, which posits a period of
accelerated expansion in the Universe's early
stages\cite{inf}\cite{PDP}. It is a useful working hypothesis that
this is the sole mechanism for generating perturbations, and it may
further be assumed to be the simplest class of inflationary model,
where the dynamics are equivalent to that of a single scalar field
$\phi$  with canonical kinetic energy slowly rolling on a potential $V(\phi)$. One may seek to verify
that this simple picture can match observations and to determine the
properties of $V(\phi)$ from the observational data. Alternatively,
more complicated models, perhaps motivated by contemporary fundamental
physics ideas, may be tested on a model-by-model basis.

Inflation generates perturbations through the amplification of quantum
fluctuations, which are stretched to astrophysical scales by the rapid
expansion. The simplest models generate two types, density
perturbations which come from fluctuations in the scalar field and its
corresponding scalar metric perturbation, and gravitational waves
which are tensor metric fluctuations. The former experience
gravitational instability and lead to structure formation, while the
latter can influence the CMB anisotropies.  Defining slow-roll
parameters, with primes indicating derivatives with respect to the
scalar field, as
$$
\epsilon = \frac{m_{{\rm Pl}}^2}{16\pi} \left( \frac{V'}{V} \right)^2 
\quad ; \quad \eta = \frac{m_{{\rm Pl}}^2}{8\pi} \frac{V''}{V} \,,
\EQN{}
$$
which should satisfy $\epsilon,|\eta| \ll 1$, the spectra can be
computed using the slow-roll approximation as
$$
\Delta^2_{\cal R}(k)  \simeq  \left. \frac{8}{3 m_{{\rm Pl}}^4} \, 
\frac{V}{\epsilon} \right|_{k=aH} \quad ; \quad
\Delta^2_{{\rm t}} (k) \simeq  \left. \frac{128}{3 m_{{\rm
Pl}}^4}  \, V \right|_{k=aH}\,.
\EQN{}
$$
In each case, the expressions on the right-hand side are to be
evaluated when the scale $k$ is equal to the Hubble radius during
inflation. The symbol `$\simeq$' here indicates use of the slow-roll
approximation, which is expected to be accurate to a few percent or
better.

From these expressions, we can compute the spectral indices\cite{LL}
$$
n_{{\rm s}} \simeq 1-6\epsilon + 2\eta \quad ; \quad n_{{\rm t}} \simeq
-2\epsilon \,. 
\EQN{}
$$
Another useful quantity is the ratio of the two spectra, defined by
$$
r \equiv \frac{\Delta^2_{{\rm t}} (k_*)}{\Delta^2_{\cal R}(k_*)} \,.
\EQN{}
$$
We have
$$
r \simeq 16 \epsilon \simeq - 8 n_{{\rm t}} \,,
\EQN{}
$$
which is known as the consistency equation.

One could consider corrections to the power-law
approximation, which we discuss later. However, for now we make the
working assumption that the spectra can be approximated by power
laws. The consistency equation shows that $r$ and $n_{{\rm t}}$ are
not independent parameters, and so the simplest inflation models give
initial conditions described by three parameters, usually taken as
$\Delta^2_{{\cal R}}$, $n_{{\rm s}}$, and $r$, all to be evaluated at some scale
$k_*$, usually the `statistical center' of the range explored by the
data.  Alternatively, one could use the parametrization $V$,
$\epsilon$, and $\eta$, all evaluated at a point on the putative
inflationary potential.
 
After the perturbations are created in the early Universe, they
undergo a complex evolution up until the time they are observed in the
present Universe.  While the perturbations are small, this can be
accurately followed using a linear theory numerical code such as
CAMB or CLASS\cite{Boltz}. This works right up to the present for the
CMB, but for density perturbations on small scales non-linear
evolution is important and can be addressed by a variety of
semi-analytical and numerical techniques. However the analysis is
made, the outcome of the evolution is in principle determined by the
cosmological model, and by the parameters describing the initial
perturbations, and hence can be used to determine them.

Of particular interest are CMB anisotropies. Both the total
intensity and two independent polarization modes are predicted to have
anisotropies. These can be described by the radiation angular power
spectra $C_\ell$ as defined in the article of Scott and Smoot in this
volume, and again provide a complete description if the density
perturbations are Gaussian.

\subsection{The standard cosmological model}
\IndexEntry{hubbleStandard}

\labelsubsection{params}

We now have most of the ingredients in place to describe the
cosmological model.  Beyond those of the previous subsections, 
we need a measure of the ionization
state of the Universe. The Universe is
known to be highly ionized at low redshifts (otherwise radiation from
distant quasars would be heavily absorbed in the ultra-violet), and
the ionized electrons can scatter microwave photons altering the
pattern of observed anisotropies. The most convenient parameter to
describe this is the optical depth to scattering $\tau$ (\ie,~the
probability that a given photon scatters once); in the approximation
of instantaneous and complete reionization, this could equivalently
be described by the redshift of reionization $z_{{\rm ion}}$. 

%\midtable{param}
%\Caption
%\IndexEntry{hubbleCosmParamA}
%The basic set of cosmological parameters. We give values (with some
%additional rounding) as obtained using a fit of a spatially-flat
%$\LAMBDA$CDM cosmology with a power-law initial spectrum to a data combination of Planck temperature anisotropies, {\it WMAP} polarization anisotropies, and small angular resolution ground-based data from ACT and SPT: Table 5, column `Planck+WP+highL' of \Ref{planckXVI}. Tensors are assumed
%zero except in quoting a limit on them. The exact values and
%uncertainties depend on both the precise data-sets used and the choice
%of parameters allowed to vary. Limits on $\OMEGA_\LAMBDA$ and $h$
%weaken if the Universe is not assumed flat.  The density perturbation
%amplitude is specified by the derived parameter $\sigma_8$.
%Uncertainties are one-sigma/68\% confidence unless otherwise stated.
%\endCaption
%\vskip 5pt
%\centerline{\vbox{
%\tabskip=0pt\offinterlineskip
%\halign  {\shortstrut#&\tabskip=0.5em plus 1em minus 0.5em% 
%               %1st column is strut
%             \lefttab{#}&           % 2nd column is text FIRST
%             \centertab{#}&           % 2nd column is text FIRST
%             \centertab{#}\tabskip=0pt\cr % 7th text FOURTH
%\tableheaddoublerule%_______________________________________
%%___________________________________________________________
%&Parameter&   Symbol & Value \cr
%\tableheadsinglerule%_______________________________________
%&Hubble parameter & $h$ & $0.673 \pm 0.012$\cr
%& Cold dark matter density & $\OMEGA_{{\rm c}}$ & $\OMEGA_{{\rm c}}
%h^2=0.1198 \pm 0.0026$ \cr 
%& Baryon density & $\OMEGA_{{\rm b}}$ & $\OMEGA_{{\rm b}} h^2 =
%0.0221\pm 0.0003$\cr 
%& Cosmological constant & $\OMEGA_\LAMBDA$ & $0.685^{+0.017}_{-0.016}$ \cr
%& Radiation density & $\OMEGA_{{\rm r}}$ & $\OMEGA_{{\rm r}} h^2 = 2.47 
%\times 10^{-5}$ \cr
%& Neutrino density & $\OMEGA_{\nu}$& See \Sec{neut} \cr
%& Density perturb. amplitude at $k=0.05$ Mpc$^{-1}$& $\ln(10^{10}\Delta_{\cal R}^2)$
% & $3.090 \pm  0.025$ \cr 
%& Density perturb. spectral index & $n_{\rm s}}$ & $0.958 \pm 0.007$\cr 
%& Tensor to scalar ratio at $k=0.002$ Mpc$^{-1}$ & $r$ & $r<0.11$ (95\% conf.) \cr
%& Ionization optical depth & $\tau$ & $0.091^{+0.014}_{-0.013}$\cr 
%& Bias parameter & $b$ & See \Sec{bias} \cr
%\tablefootdoublerule%_______________________________________
%%___________________________________________________________
%}}}
%\endtable
%

As described in \Sec{comb}, models based on these parameters
are able to give a good fit to the complete set of high-quality data
available at present, and indeed some simplification is
possible. Observations are consistent with spatial flatness, and
indeed the inflation models so far described automatically generate
negligible spatial curvature, so we can set $k = 0$; the density
parameters then must sum to unity, and so one can be eliminated. The
neutrino energy density is often not taken as an independent
parameter. Provided the neutrino sector has the standard interactions,
the neutrino energy density, while relativistic, can be related to the
photon density using thermal physics arguments, and a minimal assumption takes the neutrino mass sum to be that of the lowest mass solution to the neutrino oscillation constraints, namely $0.06$ eV. In
addition, there is no observational evidence for the existence of
tensor perturbations (though the upper limits are fairly weak), and so
$r$ could be set to zero.  This leaves seven
parameters, which is the smallest set that can usefully be compared to
the present cosmological data set. This model is referred to by various names, including
\IndexEntry{hubbleLCDM}\IndexEntry{hubbleConcord}$\LAMBDA$CDM, the 
concordance cosmology, and the standard cosmological model.

Of these parameters, only $\OMEGA_{{\rm r}}$ is accurately measured
directly.  The radiation density is dominated by the energy in the
CMB, and the COBE satellite FIRAS experiment determined its
temperature to be $T = 2.7255 \pm 0.0006 \, {\rm K}$\cite{fix},\footnote{$^\ddagger$}{Unless stated otherwise, all quoted
uncertainties in this article are one-sigma/68\% confidence and all upper limits are 95\% confidence.
Cosmological parameters sometimes have significantly non-Gaussian
uncertainties. Throughout we have rounded central values, and
especially uncertainties, from original sources in cases where they
appear to be given to excessive precision.} 
corresponding to $\OMEGA_{{\rm r}} = 2.47 \times 10^{-5} h^{-2}$. It
typically need not be varied in fitting other data. Hence the minimum number of cosmological parameters varied in fits to data is six, though as described below there may additionally be many `nuisance' parameters necessary to describe astrophysical processes influencing the data.

In addition to this minimal set, there is a range of other parameters
which might prove important in future as the data-sets further
improve, but for which there is so far no direct evidence, allowing
them to be set to a specific value for now.  We discuss various
speculative options in the next section. For completeness at this
point, we mention one other interesting parameter, the helium
fraction, which is a non-zero parameter that can affect the CMB
anisotropies at a subtle level. Fields, Molaro and Sarkar in
this volume discuss current measures of this parameter. It is usually fixed in microwave anisotropy studies,
but the data are approaching a level where allowing its variation
may become mandatory.

Most attention to date has been on parameter estimation, where a set
of parameters is chosen by hand and the aim is to constrain
them. Interest has been growing towards the higher-level inference
problem of model selection, which compares different choices of
parameter sets. Bayesian inference offers an attractive framework for
cosmological model selection, setting a tension between model
predictiveness and ability to fit the data.


\subsection{Derived parameters}

The parameter list of the previous subsection is sufficient to give a
complete description of cosmological models which agree with
observational data. However, it is not a unique parameterization, and
one could instead use parameters derived from that basic
set. Parameters which can be obtained from the set given above include
the age of the Universe, the present horizon distance, the present
neutrino background temperature, the epoch of matter--radiation
equality, the epochs of recombination and decoupling, the epoch of
transition to an accelerating Universe, the baryon-to-photon ratio,
and the baryon to dark matter density ratio.  In addition, the
physical densities of the matter components, $\OMEGA_i h^2$, are often
more useful than the density parameters.  The density perturbation
amplitude can be specified in many different ways other than the
large-scale primordial amplitude, for instance, in terms of its effect
on the CMB, or by specifying a short-scale quantity, a common choice
being the present linear-theory mass dispersion on a scale of $8 \,
h^{-1} {\rm Mpc}$, known as $\sigma_8$.

Different types of observation are sensitive to different subsets of
the full cosmological parameter set, and some are more naturally
interpreted in terms of some of the derived parameters of this
subsection than on the original base parameter set. In particular,
most types of observation feature degeneracies whereby they are unable
to separate the effects of simultaneously varying several of the base
parameters.


\section{Extensions to the standard model}
\IndexEntry{hubbleExtensions}

This section discusses some ways in which the standard model could be
extended.  At present, there is no positive evidence in favor of any
of these possibilities, which are becoming increasingly constrained by
the data, though there always remains the possibility of trace effects
at a level below present observational capability.

\subsection{More general perturbations}

The standard cosmology assumes adiabatic, Gaussian
perturbations. Adiabaticity means that all types of material in the
Universe share a common perturbation, so that if the space-time is
foliated by constant-density hypersurfaces, then all fluids and fields
are homogeneous on those slices, with the perturbations completely
described by the variation of the spatial curvature of the
slices. Gaussianity means that the initial perturbations obey Gaussian
statistics, with the amplitudes of waves of different wavenumbers
being randomly drawn from a Gaussian distribution of width given by
the power spectrum. Note that gravitational instability generates
non-Gaussianity; in this context, Gaussianity refers to a property of
the initial perturbations, before they evolve.

The simplest inflation models, based on one dynamical field, predict
adiabatic perturbations and a level of non-Gaussianity which is too
small to be detected by any experiment so far conceived. For present
data, the primordial spectra are usually assumed to be power laws.

\subsubsection{Non-power-law spectra}

For typical inflation models, it is an approximation to take the
spectra as power laws, albeit usually a good one. As data quality
improves, one might expect this approximation to come under pressure,
requiring a more accurate description of the initial spectra,
particularly for the density perturbations. In general, one can expand
$\ln \Delta_{\cal R}^2$ as
$$
\ln \Delta_{\cal R}^2(k) = \ln \Delta_{\cal R}^2(k_*) + (n_{{\rm s},*}-1) \ln 
\frac{k}{k_*} + \frac{1}{2} 
\left. \frac{dn_{{\rm s}}}{d\ln k} \right|_* \ln^2 \frac{k}{k_*} + \cdots \,,
\EQN{}
$$
where the coefficients are all evaluated at some scale $k_*$. The term
$dn_{{\rm s}}/d\ln k|_*$ is often called the running of the spectral
index\cite{KT}.  Once non-power-law spectra are
allowed, it is necessary to specify the scale $k_*$ at which
the spectral index is defined.

\subsubsection{Isocurvature perturbations}

An isocurvature perturbation is one which leaves the total density
unperturbed, while perturbing the relative amounts of different
materials. If the Universe contains $N$ fluids, there is one growing
adiabatic mode and $N-1$ growing isocurvature modes (for reviews
see \Ref{mw} and \Ref{PDP}). These can be excited, for example, in
inflationary models where there are two or more fields which acquire
dynamically-important perturbations. If one field decays to form
normal matter, while the second survives to become the dark matter,
this will generate a cold dark matter isocurvature perturbation.

In general, there are also correlations between the different modes,
and so the full set of perturbations is described by a matrix giving
the spectra and their correlations. Constraining such a general
construct is challenging, though constraints on individual modes are
beginning to become meaningful, with no evidence that any other than
the adiabatic mode must be non-zero.

\subsubsection{Seeded perturbations}

An alternative to laying down perturbations at very early epochs is
that they are seeded throughout cosmic history, for instance by
topological defects such as cosmic strings. It has long been excluded
that these are the sole original of structure, but they could
contribute part of the perturbation signal, current limits being
just a few percent\cite{planckXXV}. In particular, cosmic defects
formed in a phase transition ending inflation is a plausible scenario
for such a contribution.

\subsubsection{Non-Gaussianity}

Multi-field inflation models can also generate primordial
non-Gaussianity (reviewed, \eg, in \Ref{PDP}). The extra fields can
either be in the same sector of the underlying theory as the inflaton,
or completely separate, an interesting example of the latter being the
curvaton model\cite{curv}. Current upper limits on non-Gaussianity are
becoming stringent, but there remains strong motivation to push down those
limits and perhaps reveal trace non-Gaussianity in the data. If
non-Gaussianity is observed, its nature may favor an inflationary
origin, or a different one such as topological defects. 

\subsection{Dark matter properties}
\IndexEntry{hubbleDMA}

Dark matter properties are discussed in the article by Drees and
Gerbier in this volume.  The simplest assumption concerning the dark
matter is that it has no significant interactions with other matter,
and that its particles have a negligible velocity as far as structure
formation is concerned. Such dark matter is described as `cold,' and
candidates include the lightest supersymmetric particle, the axion,
and primordial black holes. As far as astrophysicists are concerned, a
complete specification of the relevant cold dark matter properties is
given by the density parameter $\OMEGA_{{\rm c}}$, though those
seeking to directly detect it are as interested in its interaction
properties.

Cold dark matter is the standard assumption and gives an excellent fit
to observations, except possibly on the shortest scales where there
remains some controversy concerning the structure of dwarf galaxies
and possible substructure in galaxy halos. It has long been excluded
for all the dark matter to have a large velocity dispersion, so-called
`hot' dark matter, as it does not permit galaxies to form; for thermal
relics the mass must be above about 1 keV to satisfy this constraint,
though relics produced non-thermally, such as the axion, need not obey
this limit. However, in future further parameters might need to be
introduced to describe dark matter properties relevant to
astrophysical observations. Suggestions which have been made include a
modest velocity dispersion (warm dark matter) and dark matter
self-interactions. There remains the possibility that the dark matter
is comprized of two separate components, \eg, a cold one and a hot one, an
example being if massive neutrinos have a non-negligible effect.

\subsection{Relativistic species}\IndexEntry{hubbleRelativisticSpecies}

The number of relativistic species in the young Universe (omitting photons) is denoted $N_{\rm eff}$. In the standard cosmological model only the three neutrino species contribute, and its baseline value is assumed fixed at 3.046 (the small shift from 3 is because of a slight predicted deviation from a thermal distribution\cite{man05}). However other species could contribute, for example extra neutrino species, possibly of sterile type, or massless Goldstone bosons or other scalars. It is hence interesting to study the effect of allowing this parameter to vary, and indeed although 3.046 is consistent with the data, most analyses currently suggest a somewhat higher value (\eg, \Ref{Neff}).

\subsection{Dark energy}\IndexEntry{hubbleDarkEnergy}

While the standard cosmological model given above features a
cosmological constant, in order to explain observations indicating
that the Universe is presently accelerating, further possibilities
exist under the general headings of `dark
energy' and `modified gravity'. These topics are described in detail in the article by Mortonson, Weinberg and White in this volume. This article focuses on the case of the cosmological constant, as this simple case is a good match to existing data. We note that more general treatments of dark energy/modified gravity will lead to weaker constraints on other parameters.

\subsection{Complex ionization history}

The full ionization history of the Universe is given by the ionization
fraction as a function of redshift $z$. The simplest scenario takes
the ionization to have the small residual value left after
recombination up to some redshift $z_{{\rm ion}}$, at which point the
Universe instantaneously reionizes completely. Then there is a
one-to-one correspondence between $\tau$ and $z_{{\rm ion}}$ (that
relation, however, also depending on other cosmological
parameters). An accurate treatment of this process will track separate
histories for hydrogen and helium.  While currently rapid ionization
appears to be a good approximation, as data improve a more complex
ionization history may need to be considered.

\subsection{Varying `constants'}

Variation of the fundamental constants of Nature over cosmological
times is another possible enhancement of the standard cosmology. There
is a long history of study of variation of the gravitational constant
$G_{{\rm N}}$, and more recently attention has been drawn to the possibility of
small fractional variations in the fine-structure constant. There is
presently no observational evidence for the former, which is tightly
constrained by a variety of measurements. Evidence for the latter has
been claimed from studies of spectral line shifts in quasar spectra at
redshift $z \approx 2$\cite{Webb}, but this is presently controversial
and in need of further observational study.

\subsection{Cosmic topology}

The usual hypothesis is that the Universe has the simplest topology
consistent with its geometry, for example that a flat Universe extends
forever.  Observations cannot tell us whether that is true, but they
can test the possibility of a non-trivial topology on scales up to
roughly the present Hubble scale. Extra parameters would be needed to
specify both the type and scale of the topology, for example, a
cuboidal topology would need specification of the three principal axis
lengths. At present, there is no evidence for non-trivial cosmic topology\cite{planckXXVI}.

\section{Probes}

\labelsection{obs}

The goal of the observational cosmologist is to utilize astronomical
information to derive cosmological parameters.  The transformation from
the observables to the parameters usually involves many
assumptions about the nature of the objects, as well as of the dark sector.  Below we outline the physical processes
involved in each probe, and the main recent results. The first two
subsections concern probes of the homogeneous Universe, while the
remainder consider constraints from perturbations.

In addition to statistical uncertainties
we note three sources of systematic uncertainties that will apply to the
cosmological parameters of interest: (i) due to the assumptions on the
cosmological model and its priors (\ie,~the number of assumed
cosmological parameters and their allowed range); (ii) due to the
uncertainty in the astrophysics of the objects (\eg,~light curve
fitting for supernovae or the mass--temperature relation of galaxy
clusters); and (iii) due to instrumental and observational limitations
(\eg,~the effect of `seeing' on weak gravitational lensing
measurements, or beam shape on CMB anisotropy measurements).

These systematics, the last two of which appear as `nuisance parameters', pose a challenging problem to the statistical analysis.
We attempt to fit the whole Universe with 6 to 12 parameters, but we might need to include hundreds of nuisance parameters,
some of them highly correlated with the cosmological parameters of interest (for example time-dependent 
galaxy biasing could mimic growth of mass fluctuations).  
Fortunately, there is some astrophysical prior knowledge on these effects, 
and a small number of physically-motivated free parameters 
would ideally be preferred in the cosmological parameter analysis.


\subsection{Direct measures of the Hubble constant}

In 1929, Edwin Hubble discovered the law of expansion of the Universe
by measuring distances to nearby galaxies.  The slope of the relation
between the distance and recession velocity is defined to be the
Hubble constant $H_0$.  Astronomers argued for decades on the
systematic uncertainties in various methods and derived values over
the wide range $40 \, {\rm km} \, {\rm s}^{-1} \, {\rm
Mpc}^{-1}\simlt H_0 \simlt 100 \, {\rm km} \, {\rm s}^{-1} \, {\rm
Mpc}^{-1}$.

\IndexEntry{hubbleCepheid} 
One of the most reliable results on the Hubble constant comes from the
Hubble Space Telescope Key Project\cite{freedman}.  This study used
the empirical period--luminosity relations for Cepheid variable stars
to obtain distances to 31 galaxies, and calibrated a number of
secondary distance indicators\IndexEntry{hubbleSupernovae}---Type
Ia Supernovae (SNe Ia), the Tully--Fisher relation, surface-brightness
fluctuations, and Type II Supernovae---measured over distances of
400 to 600 Mpc.  They estimated $H_0 = 72
\pm 3 \; ({\rm statistical}) \pm 7
\;({\rm systematic})\, 
{\rm km} \, {\rm s}^{-1} \, {\rm
Mpc}^{-1}$.

A recent study\cite{riess09} of over 600 Cepheids in the host galaxies
of eight recent SNe Ia, observed with an improved camera on board the
Hubble Space Telescope, was used to calibrate the magnitude--redshift
relation for 240 SNe Ia.  This yielded an even more precise figure,
$H_0 = 73.8 \pm 2.4 \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$
(including both statistical and systematic errors).  The major sources
of uncertainty in this result are due to the heavy element abundance
of the Cepheids and the distance to the fiducial nearby galaxy, the
Large Magellanic Cloud, relative to which all Cepheid distances are
measured. 

The indirect determination of $H_0$ by the {\it Planck} Collaboration\cite{planckXVI} found a lower value, 
$H_0 = 67.3 \pm 1.2 \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$.
As discussed in that paper, there is strong degeneracy of $H_0$ with other parameters, e.g. 
$\OMEGA_{\rm m}$ and the neutrino mass. 
The tension between the $H_0$ from {\it Planck}  and the traditional cosmic distance-ladder methods is under investigation. 

\subsection{Supernovae as cosmological probes}

Empirically, the peak luminosity of SNe Ia can be used as an efficient
distance indicator (\eg,~\Ref{leibundgut}), thus allowing cosmology to be constrained via the distance--redshift relation.  The favorite theoretical
explanation for SNe Ia is the thermonuclear disruption of
carbon--oxygen white dwarfs.  Although not perfect `standard candles',
it has been demonstrated that by correcting for a relation between the
light curve shape, color, and the luminosity at maximum brightness,
the dispersion of the measured luminosities can be greatly reduced.
There are several possible systematic effects which may affect the
accuracy of the use of SNe Ia as distance indicators,
\eg, evolution with redshift and interstellar extinction in
the host galaxy and in the Milky Way.

Two major studies, the Supernova Cosmology Project and the High-$z$
Supernova Search Team, found evidence for an accelerating
Universe\cite{snfirst}, interpreted as due to a cosmological constant
or a dark energy component. 
When combined with the CMB data
(which indicates flatness, \ie, $\OMEGA_{{\rm m}} +
\OMEGA_{\LAMBDA} = 1$), the best-fit values were $\OMEGA_{{\rm
m}} \approx 0.3 $ and $\OMEGA_{\LAMBDA} \approx 0.7 $.  Most results
in the literature are consistent with the $w=-1$ cosmological constant
case.  
Taking $ w=-1$, the SNLS3 team found, by combining their SNIa data with baryon acoustic oscillation (BAO) and {\it WMAP}7 data,
$\OMEGA_{\rm m} = 0.279^{+0.019}_{-0.015}$ and 
$\OMEGA_ {\LAMBDA} = 0.724^{+0.017}_{-0.016}$, including both statistical and systematic errors\cite{SNLS3}.  This
includes a correction for the recently-discovered relationship between
host galaxy mass and supernova absolute brightness.  This agrees with
earlier results\cite{kowalski}\cite{kessler}, but note the somewhat higher value for $\OMEGA_{\rm m}$ from {\it Planck} (see \Table{constraints}). 
Future experiments will
aim to set constraints on the cosmic equation of state $w(z)$.

\subsection{Cosmic microwave background}
\IndexEntry{hubbleCMB}

The physics of the CMB is described in detail by Scott and Smoot in
this volume. Before recombination, the baryons and photons are tightly
coupled, and the perturbations oscillate in the potential wells
generated primarily by the dark matter perturbations. After
decoupling, the baryons are free to collapse into those potential
wells.  The CMB carries a record of conditions at the time of
last scattering, often called primary anisotropies. In addition, it is
affected by various processes as it propagates towards us, including
the effect of a time-varying gravitational potential (the integrated
Sachs--Wolfe effect), gravitational lensing, and scattering from
ionized gas at low redshift.

\IndexEntry{hubbleCBranis}
\IndexEntry{hubbleSW}
The primary anisotropies, the integrated Sachs--Wolfe effect, and
scattering from a homogeneous distribution of ionized gas, can all be
calculated using linear perturbation theory. Available codes include
CAMB and CLASS\cite{Boltz}, the former widely used embedded within the
analysis package CosmoMC\cite{LewBrid}. Gravitational lensing is also
calculated in these codes. Secondary effects such as inhomogeneities in
the reionization process, and scattering from
gravitationally-collapsed gas
\IndexEntry{hubbleSZeldovich}(the Sunyaev--Zel'dovich (SZ) effect), 
require more complicated, and more uncertain, calculations.

The upshot is that the detailed pattern of anisotropies depends on all
of the cosmological parameters. In a typical cosmology, the anisotropy
power spectrum [usually plotted as $\ell(\ell+1)C_\ell$] features a
flat plateau at large angular scales (small $\ell$), followed by a
series of oscillatory features at higher angular scales, the first and
most prominent being at around one degree ($\ell \simeq 200$). These
features, known as acoustic peaks, represent the oscillations of the
photon--baryon fluid around the time of decoupling. Some features can
be closely related to specific parameters---for instance, the location
of the first peak probes the spatial geometry, while the relative
heights of the peaks probes the baryon density---but many other
parameters combine to determine the overall shape.

\midfigure{planckspec}
\RPPfigure{planckspec.eps,width=4.8in}{center}%
{The angular power spectrum of the CMB temperature anisotropies from
{\it Planck}, from \Ref{planckI}. Note the $x$-axis switches from logarithmic to linear at $\ell = 50$. The solid line shows the prediction from the best-fitting
$\LAMBDA$CDM model and the band indicates the cosmic variance
uncertainty. ~\colorFigAvLong ~[Figure courtesy ESA/{\it Planck} Collaboration.]  }
\IndexEntry{hubbleColorFigTwo}
\endfigure

\IndexEntry{hubblePlanck}\IndexEntry{hubbleWMAP}
The 2013 data release from the {\it Planck} satellite\cite{planckI}
has provided the most powerful results to date on
the spectrum of CMB temperature anisotropies, with a precision determination of
the temperature power spectrum to beyond $\ell = 2000$, shown
in \Fig{planckspec}. The Atacama Cosmology Telescope (ACT) and South Pole Telescope (SPT) experiments extend these results to higher angular resolution, though without full-sky coverage. The most comprehensive measurements of CMB polarization come from the {\it WMAP} satellite final (9-year) data release\cite{wmap9be}, giving the spectrum of
$E$-polarization anisotropies and the correlation spectrum between
temperature and polarization (those spectra having first been detected
by DASI\cite{DASI}). These are consistent with models based on the
parameters we have described, and provide accurate determinations of
many of those parameters\cite{planckXVI}.

The data provide an exquisite measurement of the location of the first
acoustic peak, determining the angular-diameter distance of the
last-scattering surface. In combination with other data this strongly
constrains the spatial geometry, in a manner consistent with spatial
flatness and excluding significantly-curved Universes.  CMB data also
gives a precision measurement of the age of the Universe. It gives a
baryon density consistent with, and at higher precision than, that
coming from BBN. It affirms the need for both dark matter and dark
energy.  It shows no evidence for dynamics of the dark energy, being
consistent with a pure cosmological constant ($w = -1$).
The density perturbations are consistent with a power-law primordial
spectrum, and there is no indication yet
of tensor perturbations.
\IndexEntry{hubbleReIon} 
The current best-fit for the reionization optical depth from CMB data, $\tau =
0.091$, is in line with models of how early structure
formation induces reionization.

{\it Planck} has also made the first all-sky map of the CMB lensing field, which probes the entire matter distribution in the Universe; this detection corresponds to about 25$\sigma$ and adds some additional constraining power  to the CMB-only data-sets. ACT previously announced the first detection of
gravitational lensing of the CMB from the four-point correlation of
temperature variations\cite{Das}. These measurements agree with the expected effect
in the standard cosmology.

\subsection{Galaxy clustering}
\IndexEntry{hubbleGalaxyClustering}
\labelsubsection{bias}

The power spectrum of density perturbations depends on the nature of
the dark matter.  Within the $\LAMBDA$CDM model, the power spectrum
shape depends primarily on the primordial power spectrum and on the
combination $\OMEGA_{{\rm m}} h$ which determines the horizon scale at
matter--radiation equality, with a subdominant dependence on the
baryon density.
The matter distribution is most easily probed by
observing the galaxy distribution, but this must be done with care as
the galaxies do not perfectly trace the dark matter distribution.
Rather, they are a `biased' tracer of the dark matter.  The need to
allow for such bias is emphasized by the observation that different
types of galaxies show bias with respect to each other.  In particular
scale-dependent and stochastic biasing may introduce a systematic
effect on the determination of cosmological parameters from redshift
surveys.  Prior knowledge from simulations of galaxy formation or from
gravitational lensing data could help to quantify biasing.
Furthermore, the observed 3D galaxy distribution is in redshift
space, \ie, the observed redshift is the sum of the Hubble expansion
and the line-of-sight peculiar velocity, leading to linear and
non-linear dynamical effects which also depend on the cosmological
parameters.  On the largest length scales, the galaxies are expected
to trace the location of the dark matter, except for a constant
multiplier $b$ to the power spectrum, known as the linear bias
parameter.  On scales smaller than 20 $h^{-1}$ Mpc or so, the
clustering pattern is `squashed' in the radial direction due to
coherent infall, which depends approximately on the parameter
$\beta \equiv \OMEGA_{{\rm m}}^{0.6}/b$ (on these shorter scales, more
complicated forms of biasing are not excluded by the data).  On scales
of a few $h^{-1}$ Mpc, there is an effect of elongation along the line
of sight (colloquially known as the `finger of God' effect) which
depends on the galaxy velocity dispersion.

\subsubsection{Baryonic acoustic oscillations} 
\IndexEntry{hubbleGalPwrSpec}

The power spectra of the 2-degree Field (2dF) Galaxy Redshift
Survey and the Sloan Digital Sky Survey (SDSS) are well fit by a
$\LAMBDA$CDM model and both surveys showed evidence for
BAOs\cite{eisenstein05}\cite{cole05}.  
The Baryon Oscillation Spectroscopic Survey (BOSS)  of 
Luminous Red Galaxies (LRGs) in the SDSS  found consistency with the dark energy
equation of state $w=-1$ to within $\pm 0.06$\cite{boss13}.
 Similar results for $w$ were obtained by the WiggleZ survey\cite{parkinson13}.
The BAO data from recent galaxy redshift surveys  together with SN Ia data 
are shown in a Hubble diagram in Figure 1.2. 

\midfigure{hubble_diagram}
\RPPfigure{dvlog_vs_z.eps,width=4.3in}{center}
{The cosmic distance scale with redshift. This modern version  of the  'Hubble Diagram'
combines data from SN Ia as standard candles and BAO as standard rulers in the  LRG SSDS, BOSS, 6dFGRS, and WiggleZ
galaxy surveys and from the BOSS Lyman-alpha at high redshift.
[Figure courtesy of C. Blake, based on \Ref{blake11}.]
}
~\\ %To separate figure and caption better
\IndexEntry{hubbleColorFigThree}
\endfigure


\subsubsection{Redshift distortion}

There is renewed interest in the `redshift distortion' effect.  As the
measured redshift of a galaxy is the sum of its redshift due to the
Hubble expansion and its peculiar velocity, this distortion depends on
cosmological parameters\cite{kaiser} via the perturbation growth rate in linear theory 
$f(z) = d \ln \delta /d \ln a \approx \OMEGA^\gamma(z)$, where $\gamma
\simeq 0.55$ for the $\LAMBDA$CDM model and is different for 
modified gravity models.  Recent observational
results show that by measuring $f(z)$ it is feasible to constrain $\gamma$ and rule out certain
modified gravity models\cite{guzzo}\cite{nusser11}. We note the degeneracy  of the redshift-distortion 
pattern and the geometric distortion (the so-called Alcock--Paczynski effect), 
{\it e.g.}\ as illustrated by the WiggleZ survey\cite{blake12}.

\IndexEntry{hubbleSDSS}

\subsubsection{Integrated Sachs--Wolfe effect}
 
The integrated Sachs--Wolfe (ISW) effect, described in the article by
Scott and Smoot, is the change in CMB photon energy when propagating
through the changing gravitational potential wells of developing
cosmic structures.  In linear theory, the ISW signal is expected in
universes where there is dark energy, curvature, or modified gravity.
Correlating the large-angle CMB anisotropies with very large scale
structures, first proposed in \Ref{isw1}, has provided results which 
vary from no detection of this effect to 4$\sigma$
detection\cite{tg13}\cite{planckXIX}.

\subsubsection{Limits on neutrino mass from galaxy surveys and other
probes}
\labelsubsection{neut2dF}

\IndexEntry{hubbleNuMass} 

Large-scale structure data constraints on $\OMEGA_{\nu}$
due to the neutrino free-streaming
effect\cite{lp06}.  Presently there is no clear detection, and upper
limits on neutrino mass are commonly estimated by comparing the
observed galaxy power spectrum with a four-component model of baryons,
cold dark matter, a cosmological constant, and massive neutrinos.
Such analyses also assume that the primordial power spectrum is
adiabatic, scale-invariant, and Gaussian.  Potential systematic
effects include biasing of the galaxy distribution and non-linearities
of the power spectrum.  An upper limit can also be derived from CMB
anisotropies alone, while additional cosmological data-sets can improve the results.  

Results using a photometric redshift sample of
LRGs combined with {\it WMAP}, BAO, Hubble constant and SNe Ia data gave a 95\% confidence upper limit on the total neutrino mass of 0.28eV\cite{thomas10}.
Recent spectroscopic redshift surveys, with more accurate redshifts but fewer galaxies,  yielded similar upper limits
for assumed flat $\LAMBDA$CDM model and additional data-sets:  
0.34eV from BOSS\cite{boss_nu12}
and 0.29eV from WiggleZ\cite{wigglez_nu12}.
{\it Planck} + {\it WMAP} polarization + highL CMB\cite{planckXVI} give an upper limit of 0.66eV,
and with additional BAO data 0.23eV.
The effective number of relativistic degrees of freedom is $N_{\rm eff} = 3.30 \pm 0.27$
in good agreement with the standard value $N_{\rm eff} = 3.046$.
While the latest cosmological data do not yet constrain the sum of neutrino masses to below 0.2eV,
as the lower limit on neutrino mass from
terrestrial experiments is 0.06eV, it looks promising that future
cosmological surveys will detect the neutrino mass.  

\subsection{Clusters of galaxies}

A cluster of galaxies is a large collection of galaxies held together
by their mutual gravitational attraction. The largest ones are around
$10^{15}$ Solar masses, and are the largest gravitationally-collapsed
structures in the Universe. Even at the present epoch they are
relatively rare, with only a few percent of galaxies being in
clusters.  They provide various ways to study the cosmological
parameters.

The first objects of a given kind form at the rare high peaks of the
density distribution, and if the primordial density perturbations are
Gaussian distributed, their number density is exponentially sensitive
to the size of the perturbations, and hence can strongly constrain
it. Clusters are an ideal application in the present Universe. They
are usually used to constrain the amplitude $\sigma_8$,
as a sphere of radius
$8 \, h^{-1} \, {\rm Mpc}$ contains about the right amount of
material to form a cluster. One of the most useful observations at present
are of X-ray emission from hot gas lying within the cluster, whose
temperature is typically a few keV, and which can be used to estimate
the mass of the cluster. A theoretical prediction for the mass
function of clusters can come either from semi-analytic arguments or
from numerical simulations. 
The same approach can be adopted at high redshift (which for clusters
means redshifts of order one) to attempt to measure $\sigma_8$ at an
earlier epoch.  The evolution of $\sigma_8$ is primarily driven by the
value of the matter density $\OMEGA_{{\rm m}}$, with a sub-dominant
dependence on the dark energy properties.

The {\it Planck} observations were used to produce a sample of 189 clusters 
selected by the SZ effect. 
The cluster mass function was constructed using a relation between the SZ  signal $Y$ and cluster mass $M$.
For an assumed flat $\LAMBDA$CDM model, the {\it Planck} Collaboration found
 $\sigma_8 =0.77 \pm 0.02$ and
$\OMEGA_{\rm m} = 0.29 \pm 0.02$\cite{planckXX}.
Somewhat larger values of both parameters are preferred by the {\it Planck}'s measurements of the
primary CMB anisotropies. The discrepancy might be resolved, for example, by using a different $Y$--$M$ calibration. For comparison with other results in the literature see their Fig.~10.

\subsection{Clustering in the inter-galactic medium}

It is commonly assumed, based on hydrodynamic simulations, that the
neutral hydrogen in the inter-galactic medium (IGM) can be related to
the underlying mass distribution.  It is then possible to estimate the
matter power spectrum on scales of a few megaparsecs from the
absorption observed in quasar spectra, the so-called Lyman-$\alpha$
forest.  The usual procedure is to measure the power spectrum of the
transmitted flux, and then to infer the mass power spectrum.
Photo-ionization heating by the ultraviolet background radiation and
adiabatic cooling by the expansion of the Universe combine to give a
simple power-law relation between the gas temperature and the baryon
density.  It also follows that there is a power-law relation between
the optical depth $\tau$ and $\rho_{{\rm b}}$.  Therefore, the
observed flux $F = \exp(-\tau)$ is strongly correlated with
$\rho_{{\rm b}}$, which itself traces the mass density.  The matter
and flux power spectra can be related by
$$
P_{{\rm m}}(k) = b^2(k) P_{\rm F}(k) \,,
\EQN{}
$$
where $b(k)$ is a bias function which is calibrated from simulations.
The BOSS survey has been used to detect and measure the BAO 
feature in the Lyman-$\alpha$ forest fluctuation at redshift $z=2.4$, with a result
impressively consistent with the standard $\LAMBDA$CDM model\cite{slosar13}.
The Lyman-$\alpha$  flux power spectrum has also been used to constrain the nature of dark matter,
for example constraining the amount of warm dark matter\cite{viel13}.


\subsection{Gravitational lensing}
\IndexEntry{hubbleGravLens}

Images of background galaxies are distorted by the gravitational
effect of mass variations along the line of sight.  Deep
gravitational potential wells such as galaxy clusters generate `strong
lensing', leading to arcs, arclets and multiple images, while more moderate
perturbations give rise to `weak lensing'.  Weak lensing is now widely
used to measure the mass power spectrum in selected regions of the sky
(see \Ref{lensing} for reviews).  As the signal is weak, the
image of deformed galaxy shapes (the `shear map') must be analyzed
statistically to measure the power spectrum, higher moments, and
cosmological parameters.

The shear measurements are mainly sensitive to a combination of
$\OMEGA_{{\rm m}}$ and the amplitude $\sigma_8$.  For example, the
weak-lensing signal detected by the CFHTLens Survey (over 154 sq.\ deg.\ in 5 optical bands)  yields, 
for a flat $\LAMBDA$CDM model,
$\sigma_8 (\OMEGA_{\rm m}/0.27)^{0.6} = 0.79\pm
0.03$\cite{cfhtlens13}.
Earlier results for comparison
are summarized in \Ref{lensing}. 
There are various systematic effects
in the interpretation of weak lensing, \eg, due to atmospheric
distortions during observations, the redshift distribution of the
background galaxies, the intrinsic correlation of galaxy shapes, and
non-linear modeling uncertainties.


\subsection{Peculiar velocities}

Deviations from the Hubble flow directly probe the mass perturbations
in the Universe, and hence provide a powerful probe of the dark
matter\cite{dekel}.  Peculiar velocities are deduced from the
difference between the redshift and the distance of a galaxy.  The
observational difficulty is in accurately measuring distances to
galaxies. Even the best distance indicators (\eg, the Tully--Fisher
relation) give an uncertainty of 15\% per galaxy, hence limiting the
application of the method at large distances.  Peculiar velocities are
mainly sensitive to $\OMEGA_{{\rm m}}$, not to $\OMEGA_{\LAMBDA}$ or
dark energy.  While at present cosmological parameters derived from
peculiar velocities are strongly affected by random and systematic
errors, a new generation of surveys may improve their accuracy.  Three
promising approaches are the 6dF near-infrared survey of 15,000
peculiar velocities, peculiar velocities of SNe Ia, and the
kinematic Sunyaev--Zel'dovich effect.

\section{Bringing observations together}

\labelsection{comb}

Although it contains two ingredients---dark matter and dark
energy---which have not yet been verified by laboratory experiments,
the $\LAMBDA$CDM model is almost universally accepted by cosmologists
as the best description of the present data. The approximate
values of some of the key parameters are $\OMEGA_{{\rm b}} \approx
0.05$, $\OMEGA_{{\rm c}} \approx 0.25$, $\OMEGA_{\LAMBDA} \approx
0.70$, and a Hubble constant $h \approx 0.70$. The spatial geometry is
very close to flat (and usually assumed to be precisely flat), and the
initial perturbations Gaussian, adiabatic, and nearly scale-invariant.
  
The most powerful data source is the CMB, which on its own supports
all these main tenets. Values for some parameters, as given in Ade 
\etal\cite{planckXVI} and Hinshaw \etal\cite{wmap9hi}, are reproduced
in \Table{constraints}. These particular results presume a flat Universe.
The constraints are somewhat strengthened by adding additional
data-sets such as BAO, as shown in the Table, though most of the constraining
power resides in the CMB data. We see that the {\it Planck} and {\it WMAP} constraints are similar, though with some shifts within the uncertainties. For these six-parameter fits the parameter uncertainties are also comparable; the additional precision of {\it Planck} data versus {\it WMAP} is only really apparent when considering significantly larger parameter sets.

\midtable{constraints}
\Caption
Parameter constraints reproduced from \Ref{planckXVI} (Table 5) and \Ref{wmap9hi} (Table 4), with some additional rounding.  All
columns assume the $\LAMBDA$CDM cosmology with a power-law initial
spectrum, no tensors, spatial flatness, and a cosmological constant as
dark energy. {\it Planck} take the sum of neutrino masses fixed to 0.06eV, while {\it WMAP} set it to zero. Above the line are the six parameter combinations
actually fit to the data in the {\it Planck} analysis ($\theta_{\rm MC}$ is a measure of the sound horizon at last scattering); those below the line are derived from
these. Two different data combinations including {\it Planck} are shown to highlight the
extent to which additional data improve constraints. The first column is a combination of CMB data only --- {\it Planck} temperature plus {\it WMAP} polarization data plus high-resolution data from ACT and SPT ---
while the second column adds BAO data from the SDSS, BOSS, 6dF, and WiggleZ surveys. For comparison the last column shows the final nine-year results from the {\it WMAP} satellite, combined with the same BAO data and high-resolution CMB data (which they call eCMB). Note {\it WMAP} use $\OMEGA_\LAMBDA$ directly as a fit parameter rather than $\theta_{\rm MC}$. The perturbation amplitude
$\Delta^2_{\cal R}$ is specified at the scale $0.05 \, {\rm
Mpc}^{-1}$ for {\it Planck}, but $0.002 \, {\rm Mpc}^{-1}$ for {\it WMAP}, so the spectral index $n_{{\rm s}}$ needs to be taken into account in comparing them. Uncertainties are shown at 68\% confidence.
\endCaption
\centerline{\vbox{
\tabskip=0pt\baselineskip 22pt
\halign  {\strut#&\tabskip=1em plus 1em minus 0.5em% 
               %1st column is strut
             \lefttab{#}&           % 2nd column is text FIRST
             \centertab{#}&           % 2nd column is text FIRST
             \centertab{#}&           % 3rd column is text FIRST
             \centertab{#}\tabskip=0pt\cr % 7th text FOURTH
\tableheaddoublerule%_______________________________________
%___________________________________________________________
&&   {\it Planck}+WP & {\it Planck}+WP & {\it WMAP}9+eCMB\cr
&&   +highL & +highL+BAO & +BAO\cr
\tableheadsinglerule%_______________________________________
&$\OMEGA_{{\rm b}} h^2$ & $0.02207 \pm 0.00027$ & $0.02214 \pm 0.00024$ & $0.02211 \pm 0.00034$ \cr
&$\OMEGA_{{\rm c}} h^2$ & $0.1198 \pm 0.0026$ & $0.1187 \pm 0.0017$ & $0.1162 \pm 0.0020$ \cr
&$100 \,\theta_{\rm MC}$ & $1.0413 \pm 0.0006$ & $1.0415 \pm 0.0006$ & $-$ \cr
&$n_{{\rm s}}$ & $0.958 \pm 0.007$ & $0.961 \pm 0.005$ & $0.958 \pm 0.008$\cr
&$\tau$ & $0.091^{+0.013}_{-0.014}$ & $0.092 \pm 0.013$ & $0.079^{+0.011}_{-0.012}$ \cr
&$\ln(10^{10}\Delta^2_{\cal R})$ & $3.090 \pm 0.025$ & $3.091 \pm 0.025$ & $3.212 \pm 0.029$ \cr
\tableheadsinglerule
&$h$ & $0.673 \pm 0.012$ & $0.678\pm 0.008$ & $0.688 \pm 0.008$ \cr
&$\sigma_8$ & $0.828 \pm 0.012$ & $0.826 \pm 0.012$ & $0.822^{+0.013}_{-0.014}$\cr
&$\OMEGA_{{\rm m}}$ & $0.315^{+0.016}_{-0.017}$ & $0.308 \pm 0.010$ & $0.293 \pm 0.010$\cr
&$\OMEGA_\LAMBDA$ & $0.685^{+0.017}_{-0.016}$ & $0.692 \pm 0.010$ & $0.707 \pm 0.010$ \cr
\tablefootdoublerule%_______________________________________
%___________________________________________________________
}}}
\endtable

If the assumption of spatial flatness is lifted, it turns out that
the CMB on its own only weakly constrains the spatial curvature, due to
a parameter degeneracy in the angular-diameter distance. However
inclusion of other data readily removes this. For example, inclusion of
BAO data, plus the assumption that the dark energy is
a cosmological constant, yields a constraint on
\IndexEntry{hubbleTotDen} $\OMEGA_{{\rm tot}} \equiv 
\sum \OMEGA_i + \OMEGA_\LAMBDA$ of
$\OMEGA_{{\rm tot}} = 1.0005 \pm 0.0033$\cite{planckXVI}.  Results of this
type are normally taken as justifying the restriction to flat
cosmologies.

\IndexEntry{hubbleAgeUniverse}
One parameter which is very robust is the age of the Universe, as
there is a useful coincidence that for a flat Universe the position of
the first peak is strongly correlated with the age.  The CMB data give $13.81 \pm 0.05$ Gyr (assuming flatness).  This is in good
agreement with the ages of the oldest globular clusters
and radioactive dating.
 
The baryon density $\OMEGA_{\rm b}$ is now measured with high
accuracy from CMB data alone, and is consistent
with the determination from BBN; Fields \etal\ in this volume
quote the range $0.021 \le \OMEGA_{{\rm b}} h^2
\le 0.025$ (95\% confidence).

While $\OMEGA_\LAMBDA$ is measured to be non-zero with very high
confidence, there is no evidence of evolution of the dark energy
density. Mortonson \etal\ in this volume quote the constraint $w = -1.13^{+0.13}_{-0.11}$ on a
constant equation of state from a compilation of CMB and BAO data, with the cosmological constant case $w = -1$ giving an excellent
fit to the data. Allowing more complicated forms of dark energy
weakens the limits.
  
The data provide strong support for the main predictions of the
simplest inflation models: spatial flatness and adiabatic, Gaussian,
nearly scale-invariant density perturbations. But it is disappointing
that there is no sign of primordial gravitational waves, with the CMB data compilation
providing an upper limit $r<0.11$ at 95\%
confidence\cite{planckXVI}\ (weakening to 0.26
if running is allowed). The spectral index is clearly required to be less than one by this
data, though the strength of that conclusion can weaken if additional parameters are included in the model fits.

Tests have been made for various types of non-Gaussianity, a
particular example being a parameter $f_{{\rm NL}}$ which measures a
quadratic contribution to the perturbations. Various non-gaussianity
shapes are possible (see \Ref{planckXXIV} for details), and current
constraints on the popular `local', `equilateral', and `orthogonal'
types are $ f^{{\rm local}}_{{\rm NL}} = 3 \pm 6$, $ f^{{\rm
equil}}_{{\rm NL}} = -42 \pm 75$, and $f^{{\rm ortho}}_{{\rm NL}} = -25 \pm 39$ (these look weak, but prominent non-Gaussianity
requires the product $f_{{\rm NL}}\Delta_{\cal R}$ to be large, and
$\Delta_{\cal R}$ is of order $10^{-5}$). Clearly none of these give any
indication of primordial non-gaussianity.

% This next sequence force the final section heading to the top of the page. 
% Hopefully someone better at TeX than me knows a more elegant solution.
% Two \newpage commands seem to be needed, the first to force the figure to appear. ARL
\newpage
~
\newpage

\section{Outlook for the future}

The concordance model is now well established, and there seems little
room left for any dramatic revision of this paradigm. A measure of the
strength of that statement is how difficult it has proven to formulate
convincing alternatives. 

Should there indeed be no major revision of the current paradigm, we
can expect future developments to take one of two directions. Either
the existing parameter set will continue to prove sufficient to
explain the data, with the parameters subject to ever-tightening
constraints, or it will become necessary to deploy new parameters. The
latter outcome would be very much the more interesting, offering a
route towards understanding new physical processes relevant to the
cosmological evolution. There are many possibilities on offer for
striking discoveries, for example:

\itemize
\itm The cosmological effects of a neutrino mass may be unambiguously
detected, shedding light on fundamental neutrino properties;
\itm Detection of primordial non-Gaussianities would indicate that
non-linear processes influence the perturbation generation mechanism;
\itm Detection of variation in the dark-energy density (\ie,~$w \neq
-1$) would provide much-needed experimental input into the nature of
the properties of the dark energy.
\enditemize
\noindent
These provide more than enough motivation for continued efforts to
test the cosmological model and improve its accuracy.

Over the coming years, there are a wide range of new observations
which will bring further precision to cosmological studies. Indeed,
there are far too many for us to be able to mention them all here, and
so we will just highlight a few areas.

The CMB observations will improve in several directions.  A current
frontier is the study of polarization, first detected in 2002 by DASI
and for which power spectrum measurements have now been made by
several experiments. {\it Planck} will  announce its first polarization results in 2014. Future measurements may be able to separately
detect the two modes of polarization and a number of projects are underway with this goal. 

An impressive array of dark energy surveys are already operational, under construction, or proposed, including
ground-based imaging surveys the Dark Energy Survey and
LSST, spectroscopic surveys such as MS-DESI, and 
space missions {\it Euclid} and {\it WFIRST}.  

An exciting area for the future is radio surveys of the
redshifted 21-cm line of hydrogen. Because of the intrinsic narrowness
of this line, by tuning the bandpass the emission from narrow
redshift slices of the Universe will be measured to extremely high
redshift, probing the details of the reionization process at redshifts
up to perhaps 20. LOFAR is the first instrument able to do this and is
beginning its operations. In the longer
term, the Square Kilometre Array (SKA) will take these studies to a
precision level.

The development of the first precision cosmological model is a major
achievement. However, it is important not to lose sight of the
motivation for developing such a model, which is to understand the
underlying physical processes at work governing the Universe's
evolution. On that side, progress has been much less dramatic. For
instance, there are many proposals for the nature of the dark matter,
but no consensus as to which is correct. The nature of the dark energy
remains a mystery. Even the baryon density, now measured to an
accuracy of a percent, lacks an underlying theory able to predict
it within orders of magnitude. Precision cosmology may have
arrived, but at present many key questions remain to motivate and
challenge the cosmology community.


\smallskip
\noindent{\bf References:}

\smallskip
\parindent=20pt
\ListReferences
\vfill\eject
        

\endRPPonly


==> hubble-def.tex <==
%DEFINITIONS FOR HUBBLE
\def\bolditalicx{\hbox{\bf\tenmib{x}}}
\def\bolditalick{\hbox{\bf\tenmib{k}}}
\beginRPPonly
\def\shortstrut{\vrule height 10pt depth 4pt width 0pt}
\endRPPonly
\beginDBonly
\def\shortstrut{\vrule height 9pt depth 3pt width 0pt}
\endDBonly

